Embedding and Extraction of Knowledge in Tree Ensemble Classifiers

The embedding and extraction of useful knowledge is a recent trend in machine learning applications, e.g., to supplement existing datasets that are small. Whilst, as the increasing use of machine learning models in security-critical applications, the embedding and extraction of malicious knowledge are equivalent to the notorious backdoor attack and its defence, respectively. This paper studies the embedding and extraction of knowledge in tree ensemble classifiers, and focuses on knowledge expressible with a generic form of Boolean formulas, e.g., robustness properties and backdoor attacks. For the embedding, it is required to be preservative(the original performance of the classifier is preserved), verifiable(the knowledge can be attested), and stealthy(the embedding cannot be easily detected). To facilitate this, we propose two novel, and effective, embedding algorithms, one of which is for black-box settings and the other for white-box settings.The embedding can be done in PTIME. Beyond the embedding, we develop an algorithm to extract the embedded knowledge, by reducing the problem to be solvable with an SMT (satisfiability modulo theories) solver. While this novel algorithm can successfully extract knowledge, the reduction leads to an NP computation. Therefore, if applying embedding as backdoor attacks and extraction as defence, our results suggest a complexity gap (P vs. NP) between the attack and defence when working with tree ensemble classifiers. We apply our algorithms toa diverse set of datasets to validate our conclusion extensively.

==> feedback3.tex <==
\newcommand{\marginX}{\marginnote{\huge{\quad\quad\textbf{!}\quad\quad}}}


\newcounter{point}
\setcounter{point}{0}

\newcommand{\var}{\textsf{Var}}

\newenvironment{revPoint}{
  \stepcounter{point}

  \hrule \medskip

  \noindent \textbf{\thepoint} Reviewer's comment: %\itshape
}
{
  \medskip
}

\newenvironment{reply}{\noindent \textbf{Reply}:\ }
{
  \\ \medskip
}    

\section*{Revision Letter}


\noindent First of all, we thank the editors and reviewers for their time spent on our paper. We are pleased to see reviewer 2 is satisfied with the last round's revision and appreciate his/her new comments for us to enrich the proof about the NP problem.

\subsection*{Primary Changes}

\begin{itemize}
    \item We proofread the manuscript and correct the grammar and spelling issues.
    \item We fixed the proof about NP-completeness.
\end{itemize}



In the following, we address the individual comments from the reviewer, while referring to the track-changes file for details. 

\subsection*{\bf{Reviewer \#2}}
\begin{revPoint}
\begin{quote}\small\it
There are still some grammar and spelling issues which the authors should address before publication.
\end{quote}

\begin{reply}
Thank you for the comments. we proofread the manuscript.
\end{reply}
\end{revPoint}


\begin{revPoint}
\begin{quote}\small\it
Overall, I think the proof of NP completeness is correct, but the text feels rushed and is not precise:
- you define $\kappa$ to be the most frequently occurring item in  $\kappa(x')$, but never use it.
\end{quote}
\begin{reply}
The $\kappa(x')$ is not part of the proof (and Theorem 1). Actually, the introduction of $\kappa(x')$ is to provide a practical, heuristic algorithm for the increase of $m$, while the NP computation  is for a fixed $m$. 
\end{reply}
\end{revPoint}


\begin{revPoint}
\begin{quote}\small\it
- "We may collect all possible joint paths as $\Sigma'(M, y)"$: what value does y have? In the original problem statement, these joint paths are derived from the set of inputs obtained from the outlier detection step. If you actually need all joint paths, this is an exponential step in your reduction? Please clarify this. If I understand correctly, you do not need all joint paths.
\end{quote}
\begin{reply}
As suggested in Theorem 1, the NP-completeness is for a fixed $\Sigma'(M, y)$, i.e., a fixed $y$. Therefore, in the proof, when mentioning $y$, it is the same as we need to prove in statement of Theorem 1.  
\end{reply}
\end{revPoint}

\begin{revPoint}
\begin{quote}\small\it
- you add n decision trees that always predict False, and another decision tree that always predicts True. Why do you need the last tree? If it is a tie-breaker, wouldn't (n-1) False trees suffice? You also never mention why you add these trees. I am assuming they are added to ensure that all m clauses are true when majority voting is applied.
\end{quote}
\begin{reply}
Yes, the purpose of False True trees is exactly as you expected. Thank you for pointing out that $n-1$ False trees are sufficient, we have updated this in the paper. Also, we added the following sentence for an explanation: 

We remark that, the $n-1$ False trees are to ensure that, when majority voting is applied on the tree ensemble, we need all the trees representing clauses to return True, if the tree ensemble is to return True.
\end{reply}
\end{revPoint}

\begin{revPoint}
\begin{quote}\small\it
You seem to have been inspired by the proof by Kantchelian et al.'16 (also reduction from 3-SAT, same encoding of clauses as decision trees, example is exactly the same as here http://proceedings.mlr.press/v48/kantchelian16-supp.pdf), but there is no explicit citation in that paragraph.
\end{quote}
\begin{reply}
First of all, we have cited Kantchelian et al.'16 in the paper.  For this particular proof, we note that an encoding of Boolean formula as a decision tree as described in the paper is a very typical construction, and can be found for most textbooks for artificial intelligence. Plus, the proof in Kantchelian et al.'16 is for evasion attack, not the knowledge extraction as we do in the paper. Nevertheless, we add the following remark after the proof: 

We remark that, in \cite{kantchelian2016evasion}, there is another NP-hardness proof on tree ensembles through a reduction from 3-SAT problem, but the proof is for evasion attack, different from what we prove here for knowledge extraction. Specifically, the evasion attack aims at finding an input $x'$, satisfying the constraint that $M(x') \neq M(x)$. Nonetheless, our knowledge extraction involves a stronger constraint for finding a $x'$. $x'$ should have less than $m$ features altered from original input $x$ and follow a path in given set $\Sigma'(M,y)$ at the mean time.  
\end{reply}
\end{revPoint}
